DINO Pre-training for Vision-based End-to-end Autonomous Driving

In this article, we focus on the pre-training of visual autonomous driving agents in the context of imitation learning. Current methods often rely on a classification-based pre-training, which we hypothesise to be holding back from extending capabilities of implicit image understanding. We propose pre-training the visual encoder of a driving agent using the self-distillation with no labels (DINO) method, which relies on a self-supervised learning paradigm.% and is trained on an unrelated task. Our experiments in CARLA environment in accordance with the Leaderboard benchmark reveal that the proposed pre-training is more efficient than classification-based pre-training, and is on par with the recently proposed pre-training based on visual place recognition (VPRPre).

==> bibliography.tex <==
@inproceedings{yokoyama2024vlfm,
  title={VLFM: Vision-Language Frontier Maps for Zero-Shot Semantic Navigation},
  author={Naoki Yokoyama and Sehoon Ha and Dhruv Batra and Jiuguang Wang and Bernadette Bucher},
  booktitle={International Conference on Robotics and Automation (ICRA)},
  year={2024}
}

@inproceedings{codevilla2018end,
  title={End-to-end driving via conditional imitation learning},
  author={Codevilla, Felipe and M{\"u}ller, Matthias and L{\'o}pez, Antonio and Koltun, Vladlen and Dosovitskiy, Alexey},
  booktitle={2018 IEEE International Conference on Robotics and Automation (ICRA)},
  pages={4693--4700},
  year={2018},
  organization={IEEE}
}

@article{Daniusis2021,
author={Daniu{\v{s}}is, Povilas
and Juneja, Shubham
and Valatka, Lukas
and Petkevi{\v{c}}ius, Linas},
title={Topological navigation graph framework},
journal={Autonomous Robots},
year={2021},
month={May},
day={04},
volume={45},
pages={633–646},
abstract={In this paper, we focus on the utilisation of reactive trajectory imitation controllers for goal-directed visual navigation in mobile robotics. We propose topological navigation graph (TNG) framework. TNG is an imitation-learning-based topological navigation framework for navigating through environments with intersecting trajectories. It represents the environment as a directed graph composed of perception and action modules. Each vertex of the graph corresponds to a trajectory and is represented by a trajectory identification classifier and a trajectory imitation controller. The edges of TNG correspond to intersections between trajectories and are represented by trajectory intersection recognition classifiers. Having a visually specified goal state, TNG navigates by forming a sequential composition plan of trajectory imitation controllers. We also propose to apply neural object detection architectures for the task of trajectory following by detecting direction of movement. We provide empirical evaluation of the proposed navigation framework and its components both in simulated and real-world environments and demonstrate that TNG allows us to utilise non-goal-directed, imitation-learning methods for goal-directed autonomous navigation.},
issn={1573-7527},
doi={10.1007/s10514-021-09980-x},
url={https://doi.org/10.1007/s10514-021-09980-x}
}



@inproceedings{codevilla2019exploring,
  title={Exploring the limitations of behavior cloning for autonomous driving},
  author={Codevilla, Felipe and Santana, Eder and L{\'o}pez, Antonio M and Gaidon, Adrien},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={9329--9338},
  year={2019}
}

@inproceedings{sauer2018conditional,
  title={Conditional affordance learning for driving in urban environments},
  author={Sauer, Axel and Savinov, Nikolay and Geiger, Andreas},
  booktitle={Conference on Robot Learning},
  pages={237--252},
  year={2018},
  organization={PMLR}
}

@inproceedings{chen2020learning,
  title={Learning by cheating},
  author={Chen, Dian and Zhou, Brady and Koltun, Vladlen and Kr{\"a}henb{\"u}hl, Philipp},
  booktitle={Conference on Robot Learning},
  pages={66--75},
  year={2020},
  organization={PMLR}
}

@inproceedings{toromanoff2020end,
  title={End-to-end model-free reinforcement learning for urban driving using implicit affordances},
  author={Toromanoff, Marin and Wirbel, Emilie and Moutarde, Fabien},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={7153--7162},
  year={2020}
}

@article{agarwal2021affordance,
  title={Affordance-based Reinforcement Learning for Urban Driving},
  author={Agarwal, Tanmay and Arora, Hitesh and Schneider, Jeff},
  journal={arXiv preprint arXiv:2101.05970},
  year={2021}
}

@inproceedings{karpathy2015deep,
  title={Deep visual-semantic alignments for generating image descriptions},
  author={Karpathy, Andrej and Fei-Fei, Li},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={3128--3137},
  year={2015}
}

@misc{jaegle2021perceiver,
      title={Perceiver: General Perception with Iterative Attention}, 
      author={Andrew Jaegle and others},
      year={2021},
      eprint={2103.03206},
      archivePrefix={arXiv},
      primaryClass={cs.CV}
}
@article{DBLP:journals/corr/abs-2103-03206,
  author    = {Andrew Jaegle and
               others},
  title     = {Perceiver: General Perception with Iterative Attention},
  journal   = {CoRR},
  volume    = {abs/2103.03206},
  year      = {2021},
  url       = {https://arxiv.org/abs/2103.03206},
  archivePrefix = {arXiv},
  eprint    = {2103.03206},
  timestamp = {Mon, 15 Mar 2021 17:30:55 +0100},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2103-03206.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{agarwal2021affordance,
  title={Affordance-based Reinforcement Learning for Urban Driving},
  author={Agarwal, Tanmay and Arora, Hitesh and Schneider, Jeff},
  journal={arXiv preprint arXiv:2101.05970},
  year={2021}
}

@inproceedings{dosovitskiy2017carla,
  title={CARLA: An open urban driving simulator},
  author={Dosovitskiy, Alexey and Ros, German and Codevilla, Felipe and Lopez, Antonio and Koltun, Vladlen},
  booktitle={Conference on robot learning},
  pages={1--16},
  year={2017},
  organization={PMLR}
}

@inproceedings{karpathy2014large,
  title={Large-scale video classification with convolutional neural networks},
  author={Karpathy, Andrej and others},
  booktitle={Proceedings of the IEEE conference on Computer Vision and Pattern Recognition},
  pages={1725--1732},
  year={2014}
}
@article{CGV-079,
url = {http://dx.doi.org/10.1561/0600000079},
year = {2020},
volume = {12},
journal = {Foundations and Trends® in Computer Graphics and Vision},
title = {Computer Vision for Autonomous Vehicles: Problems, Datasets and State of the Art},
doi = {10.1561/0600000079},
issn = {1572-2740},
number = {1–3},
pages = {1-308},
author = {Joel Janai and Fatma Güney and Aseem Behl and Andreas Geiger}
}

@article{osa2018algorithmic,
url = {http://dx.doi.org/10.1561/2300000053},
year = {2018},
volume = {7},
journal = {Foundations and Trends® in Robotics},
title = {An Algorithmic Perspective on Imitation Learning},
doi = {10.1561/2300000053},
issn = {1935-8253},
number = {1-2},
pages = {1-179},
author = {Takayuki Osa and Joni Pajarinen and Gerhard Neumann and J. Andrew Bagnell and Pieter Abbeel and Jan Peters}
}

@article{DAgger,
	author = {Ross, Stephane and J. Gordon, Geoffrey and Andrew Bagnell, J},
	year = {2010},
	month = {11},
	pages = {627-635},
	title = {A Reduction of Imitation Learning and Structured Prediction to No-Regret Online Learning},
	volume = {15},
	_journal = {Journal of Machine Learning Research - Proceedings Track},
  journal = {J. Mach. Learn. Res.}
}

@article{ziegler2014making,
  title={Making Bertha Drive—an Autonomous Journey on a Historic Route},
  author={Ziegler, Julius and others},
  journal={IEEE Intelligent transportation systems magazine},
  volume={6},
  number={2},
  pages={8--20},
  year={2014},
  publisher={IEEE}
}

@inproceedings{Pomerleau1988ALVINNAA,
author = {Pomerleau, Dean A.},
title = {ALVINN: An Autonomous Land Vehicle in a Neural Network},
year = {1988},
publisher = {MIT Press},
address = {Cambridge, MA, USA},
abstract = {ALVINN (Autonomous Land Vehicle In a Neural Network) is a 3-layer back-propagation network designed for the task of road following. Currently ALVINN takes images from a camera and a laser range finder as input and produces as output the direction the vehicle should travel in order to follow the road. Training has been conducted using simulated road images. Successful tests on the Carnegie Mellon autonomous navigation test vehicle indicate that the network can effectively follow real roads under certain field conditions. The representation developed to perform the task differs dramatically when the network is trained under various conditions, suggesting the possibility of a novel adaptive autonomous navigation system capable of tailoring its processing to the conditions at hand.},
booktitle = {Proceedings of the 1st International Conference on Neural Information Processing Systems},
pages = {305–313},
numpages = {9},
series = {NIPS'88}
}

@article{BojarskiTDFFGJM16,
  author    = {Bojarski, Mariusz and Del Testa, Davide and Dworakowski, Daniel and Firner, Bernhard and Flepp, Beat and Goyal, Prasoon and Jackel, Lawrence D and Monfort, Mathew and Muller, Urs and Zhang, Jiakai and others},
  title     = {End to End Learning for Self-Driving Cars},
  journal   = {CoRR},
  volume    = {abs/1604.07316},
  year      = {2016},
  archivePrefix = {arXiv},
  timestamp = {Mon, 13 Aug 2018 01:00:00 +0200},
  biburl    = {https://dblp.org/rec/bib/journals/corr/BojarskiTDFFGJM16},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@INPROCEEDINGS{8916629,
  author={Nobis, Felix and Geisslinger, Maximilian and Weber, Markus and Betz, Johannes and Lienkamp, Markus},
  booktitle={2019 Sensor Data Fusion: Trends, Solutions, Applications (SDF)}, 
  title={A Deep Learning-based Radar and Camera Sensor Fusion Architecture for Object Detection}, 
  year={2019},
  volume={},
  number={},
  pages={1-7},
  doi={10.1109/SDF.2019.8916629}}


@inproceedings{prakash2020exploringDARB,
  title={Exploring data aggregation in policy learning for vision-based urban autonomous driving},
  author={Prakash, Aditya and Behl, Aseem and Ohn-Bar, Eshed and Chitta, Kashyap and Geiger, Andreas},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={11763--11773},
  year={2020}
}

@inproceedings{zhang2017querySAFEDAgger,
    author = {Zhang, Jiakai and Cho, Kyunghyun},
    title = {Query-Efficient Imitation Learning for End-to-End Simulated Driving},
    year = {2017},
    publisher = {AAAI Press},
    abstract = {One way to approach end-to-end autonomous driving is to learn a policy that maps from a sensory input, such as an image frame from a front-facing camera, to a driving action, by imitating an expert driver, or a reference policy. This can be done by supervised learning, where a policy is tuned to minimize the difference between the predicted and ground-truth actions. A policy trained in this way however is known to suffer from unexpected behaviours due to the mismatch between the states reachable by the reference policy and trained policy. More advanced algorithms for imitation learning, such as DAgger, addresses this issue by iteratively collecting training examples from both reference and trained policies. These algorithms often require a large number of queries to a reference policy, which is undesirable as the reference policy is often expensive. In this paper, we propose an extension of the DAgger, called SafeDAgger, that is query-efficient and more suitable for end-to-end autonomous driving. We evaluate the proposed SafeDAgger in a car racing simulator and show that it indeed requires less queries to a reference policy. We observe a significant speed up in convergence, which we conjecture to be due to the effect of automated curriculum learning.},
    booktitle = {Proceedings of the Thirty-First AAAI Conference on Artificial Intelligence},
    pages = {2891–2897},
    numpages = {7},
    location = {San Francisco, California, USA},
    series = {AAAI'17}
}

@inproceedings{hu2022stp3,
  title={St-p3: End-to-end vision-based autonomous driving via spatial-temporal feature learning},
  author={Hu, Shengchao and Chen, Li and Wu, Penghao and Li, Hongyang and Yan, Junchi and Tao, Dacheng},
  booktitle={Computer Vision--ECCV 2022: 17th European Conference, Tel Aviv, Israel, October 23--27, 2022, Proceedings, Part XXXVIII},
  pages={533--549},
  year={2022},
  organization={Springer}
}

@article{chitta2022transfuser,
  title={Transfuser: Imitation with transformer-based sensor fusion for autonomous driving},
  author={Chitta, Kashyap and Prakash, Aditya and Jaeger, Bernhard and Yu, Zehao and Renz, Katrin and Geiger, Andreas},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
  year={2022},
  publisher={IEEE}
}

@article{MILE,
  title={Model-based imitation learning for urban driving},
  author={Hu, Anthony and Corrado, Gianluca and Griffiths, Nicolas and Murez, Zachary and Gurau, Corina and Yeo, Hudson and Kendall, Alex and Cipolla, Roberto and Shotton, Jamie},
  journal={Advances in Neural Information Processing Systems},
  volume={35},
  pages={20703--20716},
  year={2022}
}

@inproceedings{zhang2021endRoach,
  title={End-to-end urban driving by imitating a reinforcement learning coach},
  author={Zhang, Zhejun and Liniger, Alexander and Dai, Dengxin and Yu, Fisher and Van Gool, Luc},
  booktitle={Proceedings of the IEEE/CVF international conference on computer vision},
  pages={15222--15232},
  year={2021}
}

@article{baker2022videoVPT,
  title={Video pretraining ({VPT}): Learning to act by watching unlabeled online videos},
  author={Baker, Bowen and Akkaya, Ilge and Zhokov, Peter and Huizinga, Joost and Tang, Jie and Ecoffet, Adrien and Houghton, Brandon and Sampedro, Raul and Clune, Jeff},
  journal={Advances in Neural Information Processing Systems},
  volume={35},
  pages={24639--24654},
  year={2022}
}


@article{zhang2022actionACO,
  title={Learning to Drive by Watching YouTube videos: Action-Conditioned Contrastive Policy Pretraining},
  author={Zhang, Qihang and Peng, Zhenghao and Zhou, Bolei},
  journal={European Conference on Computer Vision (ECCV)},
  year={2022}
}

@inproceedings{wu2023policyPPgeo,
title={Policy Pre-training for Autonomous Driving via Self-supervised Geometric Modeling},
author={Penghao Wu and Li Chen and Hongyang Li and Xiaosong Jia and Junchi Yan and Yu Qiao},
booktitle={International Conference on Learning Representations},
year={2023}
}

@inproceedings{paolicelli2022learningSegVPR,
  title={Learning Semantics for Visual Place Recognition Through Multi-scale Attention},
  author={Paolicelli, Valerio and Tavera, Antonio and Masone, Carlo and Berton, Gabriele and Caputo, Barbara},
  booktitle={Image Analysis and Processing--ICIAP 2022: 21st International Conference, Lecce, Italy, May 23--27, 2022, Proceedings, Part II},
  pages={454--466},
  year={2022},
  organization={Springer}
}

@inproceedings{deng2009imagenet,
  title={Imagenet: A large-scale hierarchical image database},
  author={Deng, Jia and Dong, Wei and Socher, Richard and Li, Li-Jia and Li, Kai and Fei-Fei, Li},
  booktitle={2009 IEEE conference on computer vision and pattern recognition},
  pages={248--255},
  year={2009},
  organization={IEEE}
}

@inproceedings{wu2022trajectoryguided,
 title={Trajectory-guided Control Prediction for End-to-end Autonomous Driving: A Simple yet Strong Baseline}, 
 author={Penghao Wu and Xiaosong Jia and Li Chen and Junchi Yan and Hongyang Li and Yu Qiao},
 booktitle={NeurIPS},
 year={2022},
}

@ARTICLE{EndtoendSurvey,
author={Tampuu, Ardi and Matiisen, Tambet and Semikin, Maksym and Fishman, Dmytro and Muhammad, Naveed},
journal={IEEE Transactions on Neural Networks and Learning Systems}, 
title={A Survey of End-to-End Driving: Architectures and Training Methods}, 
year={2022},
volume={33},
number={4},
pages={1364-1384},
doi={10.1109/TNNLS.2020.3043505}}

@inproceedings{Resnet,
  title={Deep residual learning for image recognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={770--778},
  year={2016}
}

@article{paszke2019pytorch,
  title={Pytorch: An imperative style, high-performance deep learning library},
  author={Paszke, Adam and Gross, Sam and Massa, Francisco and Lerer, Adam and Bradbury, James and Chanan, Gregory and Killeen, Trevor and Lin, Zeming and Gimelshein, Natalia and Antiga, Luca and others},
  journal={Advances in neural information processing systems},
  volume={32},
  year={2019}
}

@inproceedings{ImageNetTransferBetter,
  title={Do better imagenet models transfer better?},
  author={Kornblith, Simon and Shlens, Jonathon and Le, Quoc V},
  booktitle={Proceedings of the IEEE/CVF conference on computer vision and pattern recognition},
  pages={2661--2671},
  year={2019}
}

@inproceedings{Taskonomy,
  title={Taskonomy: Disentangling task transfer learning},
  author={Zamir, Amir R and Sax, Alexander and Shen, William and Guibas, Leonidas J and Malik, Jitendra and Savarese, Silvio},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={3712--3722},
  year={2018}
}

@inproceedings{coco,
  title={Microsoft {COCO}: Common objects in context},
  author={Lin, Tsung-Yi and Maire, Michael and Belongie, Serge and Hays, James and Perona, Pietro and Ramanan, Deva and Doll{\'a}r, Piotr and Zitnick, C Lawrence},
  booktitle={Computer Vision--ECCV 2014: 13th European Conference, Zurich, Switzerland, September 6-12, 2014, Proceedings, Part V 13},
  pages={740--755},
  year={2014},
  organization={Springer}
}


@inproceedings{ObjectDetection,
  title={Speed/accuracy trade-offs for modern convolutional object detectors},
  author={Huang, Jonathan and Rathod, Vivek and Sun, Chen and Zhu, Menglong and Korattikara, Anoop and Fathi, Alireza and Fischer, Ian and Wojna, Zbigniew and Song, Yang and Guadarrama, Sergio and others},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={7310--7311},
  year={2017}
}

@inproceedings{ImageSegmentation,
  title={Mask {R-CNN}},
  author={He, Kaiming and Gkioxari, Georgia and Doll{\'a}r, Piotr and Girshick, Ross},
  booktitle={Proceedings of the IEEE international conference on computer vision},
  pages={2961--2969},
  year={2017}
}

@inproceedings{GPT3,
 author = {Brown, Tom and Mann, Benjamin and Ryder, Nick and Subbiah, Melanie and Kaplan, Jared D and Dhariwal, Prafulla and Neelakantan, Arvind and Shyam, Pranav and Sastry, Girish and Askell, Amanda and Agarwal, Sandhini and Herbert-Voss, Ariel and Krueger, Gretchen and Henighan, Tom and Child, Rewon and Ramesh, Aditya and Ziegler, Daniel and Wu, Jeffrey and Winter, Clemens and Hesse, Chris and Chen, Mark and Sigler, Eric and Litwin, Mateusz and Gray, Scott and Chess, Benjamin and Clark, Jack and Berner, Christopher and McCandlish, Sam and Radford, Alec and Sutskever, Ilya and Amodei, Dario},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {H. Larochelle and M. Ranzato and R. Hadsell and M.F. Balcan and H. Lin},
 pages = {1877--1901},
 publisher = {Curran Associates, Inc.},
 title = {Language Models are Few-Shot Learners},
 url = {https://proceedings.neurips.cc/paper_files/paper/2020/file/1457c0d6bfcb4967418bfb8ac142f64a-Paper.pdf},
 volume = {33},
 year = {2020}
}


@article{chen2023e2esurvey,
  title={End-to-end Autonomous Driving: Challenges and Frontiers},
  author={Chen, Li and Wu, Penghao and Chitta, Kashyap and Jaeger, Bernhard and Geiger, Andreas and Li, Hongyang},
  journal={arXiv},
  volume={2306.16927},
  year={2023}
}

@inproceedings{hu2023_uniad,
 title={Planning-oriented Autonomous Driving}, 
 author={Yihan Hu and Jiazhi Yang and Li Chen and Keyu Li and Chonghao Sima and Xizhou Zhu and Siqi Chai and Senyao Du and Tianwei Lin and Wenhai Wang and Lewei Lu and Xiaosong Jia and Qiang Liu and Jifeng Dai and Yu Qiao and Hongyang Li},
 booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
 year={2023},
}

@ARTICLE{VPRpretrain,
  author={Juneja, Shubham and Daniušis, Povilas and Marcinkevičius, Virginijus},
  journal={IEEE Access}, 
  title={Visual Place Recognition Pre-Training for End-to-End Trained Autonomous Driving Agent}, 
  year={2023},
  volume={11},
  number={},
  pages={128421-128428},
  keywords={Task analysis;Training;Meteorology;Lighting;Autonomous vehicles;Visualization;Learning systems;Autonomous driving;Visualization;Imitation learning;autonomous driving;agents;self-driving cars;deep learning;pre-training},
  doi={10.1109/ACCESS.2023.3331678}}

@inproceedings{dinoV1,
  title={Emerging Properties in Self-Supervised Vision Transformers},
  author={Caron, Mathilde and Touvron, Hugo and Misra, Ishan and J\'egou, Herv\'e  and Mairal, Julien and Bojanowski, Piotr and Joulin, Armand},
  booktitle={Proceedings of the International Conference on Computer Vision (ICCV)},
  year={2021}
}

 @misc{CILplus,
 title={Scaling Vision-based End-to-End Driving with Multi-View Attention Learning},
 author={Yi Xiao and Felipe Codevilla and Diego Porres and Antonio M. Lopez},
 year={2023},
 eprint={2302.03198},
 archivePrefix={arXiv},
 primaryClass={cs.CV}
 }

@article{PerceiverSelf,
    author={Juneja, Shubham and Daniušis, Povilas and Marcinkevičius, Virginijus},
    title = {Combining Multiple Modalities with Perceiver in Imitation-based Urban Driving},
    journal = {ALLSENSORS 2021, The Sixth International Conference on Advances in Sensors, Actuators, Metering and Sensing},
    year = {2021}
}

@article{MultimodelYiXao,
author = {Xiao, Yi and Codevilla, Felipe and Gurram, Akhil and Urfalioglu, Onay and L\'{o}pez, Antonio M.},
title = {Multimodal End-to-End Autonomous Driving},
year = {2022},
issue_date = {Jan. 2022},
publisher = {IEEE Press},
volume = {23},
number = {1},
issn = {1524-9050},
url = {https://doi.org/10.1109/TITS.2020.3013234},
doi = {10.1109/TITS.2020.3013234},
abstract = {A crucial component of an autonomous vehicle (AV) is the artificial intelligence (AI) is able to drive towards a desired destination. Today, there are different paradigms addressing the development of AI drivers. On the one hand, we find modular pipelines, which divide the driving task into sub-tasks such as perception and maneuver planning and control. On the other hand, we find end-to-end driving approaches that try to learn a direct mapping from input raw sensor data to vehicle control signals. The later are relatively less studied, but are gaining popularity since they are less demanding in terms of sensor data annotation. This paper focuses on end-to-end autonomous driving. So far, most proposals relying on this paradigm assume RGB images as input sensor data. However, AVs will not be equipped only with cameras, but also with active sensors providing accurate depth information (<italic>e.g.</italic>, LiDARs). Accordingly, this paper analyses whether combining RGB and depth modalities, <italic>i.e.</italic> using RGBD data, produces better end-to-end AI drivers than relying on a single modality. We consider multimodality based on early, mid and late fusion schemes, both in multisensory and single-sensor (monocular depth estimation) settings. Using the CARLA simulator and conditional imitation learning (CIL), we show how, indeed, early fusion multimodality outperforms single-modality.},
journal = {Trans. Intell. Transport. Sys.},
month = {jan},
pages = {537–547},
numpages = {11}
}

@inproceedings{he2020momentum,
  title={Momentum contrast for unsupervised visual representation learning},
  author={He, Kaiming and Fan, Haoqi and Wu, Yuxin and Xie, Saining and Girshick, Ross},
  booktitle={Proceedings of the IEEE/CVF conference on computer vision and pattern recognition},
  pages={9729--9738},
  year={2020}
}

@article{caron2020unsupervised,
  title={Unsupervised learning of visual features by contrasting cluster assignments},
  author={Caron, Mathilde and Misra, Ishan and Mairal, Julien and Goyal, Priya and Bojanowski, Piotr and Joulin, Armand},
  journal={Advances in neural information processing systems},
  volume={33},
  pages={9912--9924},
  year={2020}
}

@inproceedings{jia2023thinktwice,
  title={Think twice before driving: Towards scalable decoders for end-to-end autonomous driving},
  author={Jia, Xiaosong and Wu, Penghao and Chen, Li and Xie, Jiangwei and He, Conghui and Yan, Junchi and Li, Hongyang},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={21983--21994},
  year={2023}
}

@article{vaswani2017attention,
  title={Attention is all you need},
  author={Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N and Kaiser, {\L}ukasz and Polosukhin, Illia},
  journal={Advances in neural information processing systems},
  volume={30},
  year={2017}
}

@article{minaee2024LLM,
  title={Large language models: A survey},
  author={Minaee, Shervin and Mikolov, Tomas and Nikzad, Narjes and Chenaghlu, Meysam and Socher, Richard and Amatriain, Xavier and Gao, Jianfeng},
  journal={arXiv preprint arXiv:2402.06196},
  year={2024}
}
